Checking Satisfiability by Dependency Sequents

We introduce a new algorithm for checking satisfiability based on a calculus of Dependency sequents (D-sequents). Given a CNF formula F(X), a D-sequent is a record stating that under a partial assignment a set of variables of X is redundant in formula \exists{X}[F]. The D-sequent calculus is based on operation join that forms a new D-sequent from two existing D-sequents. The new algorithm solves the quantified version of SAT. That is, given a satisfiable formula F, it, in general, does not produce an assignment satisfying F. The new algorithm is called DS-QSAT where DS stands for Dependency Sequent and Q for Quantified. Importantly, a DPLL-like procedure is only a special case of DS-QSAT where a very restricted kind of D-sequents is used. We argue that this restriction a) adversely affects scalability of SAT-solvers and b) is caused by looking for an explicit satisfying assignment rather than just proving satisfiability. We give experimental results substantiating these claims.

==> undo.tex <==
\begin{example}
$\pnt{q}=(x_1=0,x_2=1,x_3=0,x_5=0)$.  The only clauses of $F$ containing the positive literal of $x_5$ are
 $C_1=x_5 \vee x_7$ and $C_2=x_5 \vee \overline{x}_1$.

Let $S_1$ and $S_2$ be the only valid D-sequents where $S_1$ is equal to $(x_5=0) \rightarrow \s{x_{10}}$
and $S_2$ is equal to $(x_3=0) \rightarrow \s{x_7}$.

Suppose, $x_5=0$ is the first assignment (left branch). The one can skip the right branch by performing
the following steps.   The D-sequent $(x_1=0,x_3=0) \rightarrow \s{x_5}$ is generated for the branching variable $x_5$.
The D-sequent $S_1$ is updated to $(x_1=0,x_3=0) \rightarrow \s{x_{10}}$.
\end{example}

-------------
%
%  The other D-sequents
%
\begin{proposition}
\end{proposition}
\begin{proof}
\end{proof}
-------
 Then there is a \s{v}-boundary point 
of \cof{F}{r} that is removable in $F$.
------
(recall
that the value of $v$ in \pnt{e} is 0).
---------------
The first column of Table~\ref{tbl:compos_form_stat2} recalls the number of variables of the formulas (in thousands). 
-----------
The computation of D-sequent for the branching variable
$v$ and recomputation of D-sequents of $\DS_0$ is described below. The correctness of D-sequents
produced by SRB technque  is proved in Propositions~\ref{prop:SRB1} and ~\ref{prop:SRB2}. 
------------
because $v$ is virtually redundant in \cof{F}{r} (see Subsection ~\ref{subsec:virt_redund}).
------------
\item eventually the correct D-sequent $\emptyset \rightarrow \s{v}$ is derived for every variable $v \in X$, which 
means  derivation of  D-sequent $\emptyset \rightarrow X$.k
---------
*)\> $S_1,S_2,S_4$ are D-sequents of \\
\> monotone variables \\
*)\> $S_3$ is obtained by joining \\
\> $S_1,S_2$ at variable $x_4$ \\
*)\> $S_5$ is derived due to $C_9(\pnt{q})=0$ \\
\> where \pnt{q} = $(x_1=0,x_2=0)$ \\

